CrossNet: An End-to-end Reference-based Super Resolution Network using Cross-scale Warping

The Reference-based Super-resolution (RefSR) super-resolves a low-resolution (LR) image given an external high-resolution (HR) reference image, where the reference image and LR image share similar viewpoint but with significant resolution gap x8. Existing RefSR methods work in a cascaded way such as patch matching followed by synthesis pipeline with two independently defined objective functions, leading to the inter-patch misalignment, grid effect and inefficient optimization. To resolve these issues, we present CrossNet, an end-to-end and fully-convolutional deep neural network using cross-scale warping. Our network contains image encoders, cross-scale warping layers, and fusion decoder: the encoder serves to extract multi-scale features from both the LR and the reference images; the cross-scale warping layers spatially aligns the reference feature map with the LR feature map; the decoder finally aggregates feature maps from both domains to synthesize the HR output. Using cross-scale warping, our network is able to perform spatial alignment at pixel-level in an end-to-end fashion, which improves the existing schemes both in precision (around 2dB-4dB) and efficiency (more than 100 times faster).

==> section/model.tex <==
\section{Approach}

\begin{figure}
	\centering
	\includegraphics[width=1.0\textwidth]{figures/main.pdf}
	\caption{(a): network structure of our proposed EWD-SRNet, (b): an image warping + synthesis pipeline for comparison }
	\label{fig:model}
\end{figure}

Figure \ref{fig:model} summarizes the structure of our proposed EWD-SRNet (left) and compares it against an image warping + fusion pipeline (right) which resembles the network structure of \cite{task_flow} \cite{LFVideo}. Our key observations for EWD-SRNet are: 
First, performing warping at only the finest scale slowdowns the convergence, as the flow-field vector is updated by only searching image (or feature) contents withing 1 block-matching distance from that vector. To enlarge the content searching space, we instead utilizes flow-fields from lower scales to higher scales to perform a sequential of warping operations. Second, performing warping and fusion on the raw-images domain is not optimal, because the raw LR and reference images do not specifically provide complementary and task oriented informations for fusion. Conversely, our model extract multi-scale feature maps from the LR image and reference image for feature-based warping and fusion.
Finally, we proposed an decoder for feature fusion and synthesis using U-Net structure. Our decoder contains multiple skip connections between the flow-field estimator and the fusion module, which allows gradient to propagate easier from latter to former. Comparing to the image warping + fusion counterpart, our proposed model can be directly trained without pre-training the flow-field estimator.

%Finally, the training dynamic of such model is further complicated by the fact that t update of the flow-estimator relies on the . training dynamic of such model is further complicated by the fact that the update of the flow-estimator relies on the. flow-field estimator is also hindered by the training . The training is complicated by the fact that the inputs to each layer are affected by the parameters of all preceding layers

\subsection{Multi-scale Flow-field Estimator}
As shown on the top of Figure \ref{fig:model}(a), given an bicubic upsampled LR image and its corresponding reference image, we adopt the widely used the FlowNetS \cite{FlowNet} as our multi-scale flow-field estimator. To improve the FlowNetS, we made several modifications: firstly, the activation function of FlowNetS is change from ReLU to SELU \cite{SELU} which considerably improves the model convergence; on the top of that, we additionally replace the final $\times 4$ bilinear upsampling layer of FlownetS with two deconvolution layer following skip connection layers for up-sampling the flow-field twice. The additional upsampling layers allows our modified model to output flow-field with much finner definition.

\subsection{Reference Image Encoder}
Given the reference image $I_R$, we designed a reference encoder to extract reference feature maps at 4 scales. Specifically, we convolves the raw reference images with 64 $5 \times 5$ filters with stride 1 to extract feature map at scale $0$. After that, we repeatedly convolves the feature map at scale $i-1$ (for $0 < i \le 3$) with with 64 $5 \times 5$ filters with stride 2 to extract feature map at scale $i$:

%\begin{equation}
\begin{eqnarray}
	F^{(0)}_R &=& \delta(\boldsymbol{W}^{(0)}_R \ast I_R + \boldsymbol{b}^{(0)}_R), \\
	F^{(i)}_R &=& \delta(\boldsymbol{W}^{(i)}_R \ast F^{(i-1)}_R + \boldsymbol{b}^{(i)}_R) {\Downarrow_2}, ~ i = {1,2,3}.
\end{eqnarray}
%\end{equation}

\subsection{LR Image Encoder}
Given the LR image, we utilize an single-image SR (SISR) approach \cite{MDSR} to upsample the LR image to the same scale as the reference image. After that, an LR image encoder with the exact structure of the reference image encoder are employed to extract the LR image features maps. However, we allow the LR image encoder and the reference image encoder to learn different weights, which help the two sets of features to complement each other. 

%\begin{equation}{l}
\begin{eqnarray}
SR_L &=& SISR(I_L), \\
F^{(0)}_L &=& \delta(\boldsymbol{W}^{(0)}_L \ast SR_L + \boldsymbol{b}^{(0)}_L), \\
F^{(i)}_L &=& \delta(\boldsymbol{W}^{(i)}_L \ast F^{(i-1)}_L + \boldsymbol{b}^{(i)}_L) {\Downarrow_2}, ~ i = {1,2,3}.
\end{eqnarray}
%\end{equation}

Utilizing independent SISR approaches (such as \cite{MDSR} ) to encode LR image has two advantages: First, the SISR approaches that are validated on large-scale external datasets helps the LR image encoder to generalize better on unseen scenes; second, new state-of-the-art SISR approaches can be easily integrated into our system to improve performance without changing our network structures.

\subsection{Flow Estimator}
We applied a modified FlownetS \cite{FlowNet} as our flow estimator. Specifically, to increase the flow precision, we replace the final $\times4$ bilinear upscaling layer of FlownetS with two deconvolution layer using skip connection for $\times2$ upscaling. The modified flow estimator is used to generate the multi-scale flow.

\begin{eqnarray}
\{V^{(3)}, V^{(2)}, V^{(1)}, V^{(0)}\} = {Flow}(I_L, I_R)
\end{eqnarray}


\subsection{Decoder using Fusion}
After extracting multi-scale image features and the corresponding flow-fields at different scales, we warp the reference feature using backward warping at every scales. 

\begin{eqnarray}
	F^{(i)}_{Rw} = warp(F^{(i)}_R, V^{(i))}), ~ i = {0,1,2,3}.
\end{eqnarray}


After that, a U-Net like decoder is proposed to perform fusion and SR synthesis. Specifically, the warped features and the LR image features at scale $i$ (for $0 < i \le 3$), as well as the decoder feature from scale $i-1$ are concatenated following a deconvolution layer with 64 $4 \times 4$ filters and stride 2 to generate decoder features at scale $i$. 

\begin{eqnarray}
F^{(3)}_{d} &=& \delta(\boldsymbol{W}^{(3)}_{d} \star (F^{(3)}_L, F^{(3)}_{Rw}) + \boldsymbol{b}^{(3)}_{d}), \\
F^{(i)}_{d} &=& \delta(\boldsymbol{W}^{(i)}_{d} \star (F^{(i+1)}_L, F^{(i+1)}_{Rw}, F^{(i+1)}_{d}) + \boldsymbol{b}^{(i)}_d), ~ i = {2,1,0}.
\end{eqnarray}

After generating the decoder feature at scale $0$, 3 additional convolution layers with filter sizes $5 \times 5$ and filter number $\{64,64,3\}$ are added to synthesis the SR output. 

\begin{eqnarray}
F^{}_{1} &=& \delta(\boldsymbol{W}^{(0)}_p \ast F^{(i)}_{d} + \boldsymbol{b}^{(0)}_p), \\
F^{}_{2} &=& \delta(\boldsymbol{W}^{(0)}_p \ast F^{}_{1} + \boldsymbol{b}^{(0)}_p),	\\
I_p &=& \delta(\boldsymbol{W}^{(0)}_p \ast F^{}_{2} + \boldsymbol{b}^{(0)}_p).
\end{eqnarray}

\subsection{Loss Function}
Our network can be directly trained to synthesis the SR output. Given the reference image $I_{R}$, the LR image $I_{L}$, the network prediction $I_{p}$ and the ground truth image $I_{H}$, the loss function can be written as:

\begin{eqnarray}
	\mathcal{L} = \frac{1}{N} \sum_{i=1}^{N} \sum_{s} \rho (I_{H}^{(i)}(s) - I_{p}^{(i)}(s) ),
\end{eqnarray}

where $\rho(x)=\sqrt{x^2+0.001^2}$ is the Charbonnier penalty function \cite{Charbonnier}, N is the number of samples, $i$ and $s$ iterate over training samples and spatial locations respectively.




==> section/model_v2.tex <==
\section{Approach}

\begin{figure}
	\centering
	\includegraphics[width=1.0\textwidth]{figures/main.pdf}
	\caption{(a): network structure of the proposed EWD-SRNet, (b): an image warping + synthesis pipeline for comparison. \fang{remove the sub-caption of sub-figure, and exchange the order of two figures}}
	\label{fig:model}
\end{figure}

When we investigate the conventional cascaded `image warping + synthesis' pipeline (in Fig. \ref{fig:model}(a)) which resembles the network structure of \cite{task_flow} \cite{LFVideo}, our key observations are: 1) performing warping at the finest scale slowdowns the convergence, as the flow-field vector is updated by only searching image (or feature) contents within 1 block-matching distance from the vector. 2) performing warping and fusion on the raw-images directly is not optimal, because the raw LR and reference images do not explicitly provide complementary informations for fusion. 

For the former issue, we propose to utilize flow-fields from lower scales to higher scales to perform a sequential of warping operations, so as to enlarge the content searching space. For the latter one, our model will extract multi-scale feature maps from the LR image and reference image for feature-based warping and fusion, instead of using raw images directly. We further propose an decoder for feature fusion and synthesis using U-Net structure. Our decoder contains multiple skip connections between the flow-field estimator and the fusion module, which allows gradient to propagate easier from latter to former. Comparing to the cascaded counterpart, {\bf our proposed model can be directly trained without pre-training the flow-field estimator}. Fig. \ref{fig:model}(b) summarizes the structure of our proposed EWD-SRNet. The major modules, i.e., encoder, estimator and decoder, are elaborated as follows.

%Finally, the training dynamic of such model is further complicated by the fact that t update of the flow-estimator relies on the . training dynamic of such model is further complicated by the fact that the update of the flow-estimator relies on the. flow-field estimator is also hindered by the training . The training is complicated by the fact that the inputs to each layer are affected by the parameters of all preceding layers



\subsection{Encoder}

Reference Image Encoder: Given the reference image $I_R$, we design a reference image encoder to extract reference feature maps at 4 scales. Specifically, we convolve the raw reference images with 64 filters (of size $5 \times 5$) with stride 1 to extract feature map at scale $0$. After that, we repeatedly convolve the feature map at the scale $i-1$ (for $0 < i \le 3$) with 64 filters (of size $5 \times 5$) with stride 2 to extract feature map at scale $i$. Such operations can be represented as
\begin{equation}
\begin{array}{rl}
	F^{(0)}_R &= \delta(\boldsymbol{W}^{(0)}_R \ast I_R + \boldsymbol{b}^{(0)}_R), \\\\
	F^{(i)}_R &= \delta(\boldsymbol{W}^{(i)}_R \ast F^{(i-1)}_R + \boldsymbol{b}^{(i)}_R) {\Downarrow_2}, ~ i = {1,2,3},
	\end{array}
\end{equation}
where XXXXXXXX \fang{explain the equation and introduce the notations}.

LR Image Encoder: Given the LR image $I_L$, we utilize the representative Single-Image SR (SISR) approach \cite{MDSR} to upsample the LR image to the same scale as the reference image. After that, an LR image encoder with the exact structure of the reference image encoder is employed to extract the LR image features maps. Particularly, we allow the LR image encoder and the reference image encoder to learn different weights, which helps the two sets of features to complement each other. 
%\begin{eqnarray}
%SR_L &=& SISR(I_L), \\
%F^{(0)}_L &=& \delta(\boldsymbol{W}^{(0)}_L \ast SR_L + \boldsymbol{b}^{(0)}_L), \\
%F^{(i)}_L &=& \delta(\boldsymbol{W}^{(i)}_L \ast F^{(i-1)}_L + \boldsymbol{b}^{(i)}_L) {\Downarrow_2}, ~ i = {1,2,3}.
%\end{eqnarray}

Note that utilizing independent SISR approaches (such as \cite{MDSR} ) to encode LR image owns two advantages. First, the SISR approaches that are validated on large-scale external datasets help the LR image encoder to generalize better on unseen scenes. Second, new state-of-the-art SISR approaches can be easily integrated into our system to improve performance without changing our network structures.


\subsection{Multi-scale Flow-field Estimator}
As shown on the top of Fig. \ref{fig:model}(a), given an bicubic upsampled LR image\footnote{It is observed by \cite{SS-Net} that SISR upsampled images are not suitable for correspondence inference, as some spatial clues for correspondence matching are lost during the SISR process.} \fang{it is confusing here, why do you mention bicubic??????} and its corresponding reference image, we adopt and further improve the widely used FlowNetS \cite{FlowNet} as our multi-scale flow-field estimator. Specifically, the improvements are: 1) the activation function of FlowNetS is changed from ReLU to SELU \cite{SELU} which considerably improves the model convergence, 2) we replace the final $\times 4$ bilinear upsampling layer of FlownetS with two deconvolution layer following skip connection layers for up-sampling the flow-field twice. Such additional upsampling layers allow our modified model to output flow-field with much finer definition. The modified flow estimator works to generate the multi-scale flow as follows.
\begin{eqnarray}
\{V^{(3)}, V^{(2)}, V^{(1)}, V^{(0)}\} = {Flow}(I_L, I_R).
\end{eqnarray}

\fang{add more discussion about multi-scale property}

\subsection{Decoder}
After extracting multi-scale image features and the corresponding flow-fields at different scales, we warp the reference feature using backward warping at every scales,
\begin{eqnarray}
	\hat{F}^{(i)}_{R} = warp(F^{(i)}_R, V^{(i))}), ~ i = {0,1,2,3},
\end{eqnarray}
where $\hat{F}^{(i)}_{R}$ denotes XXXXXXXXXX. \fang{explain the equation and define the notations} 

\fang{you did not explain why using backward warping????????????}

Then, a U-Net like decoder is proposed to perform fusion and SR synthesis. Specifically, the warped features and the LR image features at scale $i$ (for $0 < i \le 3$), as well as the decoder feature from scale $i-1$ are concatenated following a deconvolution layer with 64 filters (of size $4 \times 4$) and stride 2 to generate decoder features at scale $i$, 
\begin{equation}
\begin{array}{rl}
F^{(3)}_{d} &= \delta(\boldsymbol{W}^{(3)}_{d} \star (F^{(3)}_L, F^{(3)}_{Rw}) + \boldsymbol{b}^{(3)}_{d}), \\\\
F^{(i)}_{d} &= \delta(\boldsymbol{W}^{(i)}_{d} \star (F^{(i+1)}_L, F^{(i+1)}_{Rw}, F^{(i+1)}_{d}) + \boldsymbol{b}^{(i)}_d), ~ i = {2,1,0}.
\end{array}
\end{equation}

After generating the decoder feature at scale $0$, three additional convolution layers with filter sizes $5 \times 5$ and filter number $\{64, 64, 3\}$ are added to synthesize the SR output,
\begin{equation}
\begin{array}{lll}
F^{}_{1} & = &\delta(\boldsymbol{W}^{(0)}_p \ast F^{(i)}_{d} + \boldsymbol{b}^{(0)}_p), \\
F^{}_{2} &=& \delta(\boldsymbol{W}^{(0)}_p \ast F^{}_{1} + \boldsymbol{b}^{(0)}_p),	\\
I_p &=& \delta(\boldsymbol{W}^{(0)}_p \ast F^{}_{2} + \boldsymbol{b}^{(0)}_p).
\end{array}
\end{equation}

\subsection{Loss Function}
Our network can be directly trained to synthesize the SR output. Given the reference image $I_{R}$, the LR image $I_{L}$, the network prediction $I_{p}$, and the ground truth high-resolution image $I_{H}$, the loss function can be written as
\begin{eqnarray}
	\mathcal{L} = \frac{1}{N} \sum_{i=1}^{N} \sum_{s} \rho (I_{H}^{(i)}(s) - I_{p}^{(i)}(s) ),
\end{eqnarray}
where $\rho(x)=\sqrt{x^2+0.001^2}$ is the Charbonnier penalty function \cite{Charbonnier}, N is the number of samples, $i$ and $s$ iterate over training samples and spatial locations, respectively.



